Graph Attention Networks with Positional Embeddings

Graph Neural Networks (GNNs) are deep learning methods which provide the current state of the art performance in node classification tasks. GNNs often assume homophily -- neighboring nodes having similar features and labels--, and therefore may not be at their full potential when dealing with non-homophilic graphs. In this work, we focus on addressing this limitation and enable Graph Attention Networks (GAT), a commonly used variant of GNNs, to explore the structural information within each graph locality. Inspired by the positional encoding in the Transformers, we propose a framework, termed Graph Attentional Networks with Positional Embeddings (GAT-POS), to enhance GATs with positional embeddings which capture structural and positional information of the nodes in the graph. In this framework, the positional embeddings are learned by a model predictive of the graph context, plugged into an enhanced GAT architecture, which is able to leverage both the positional and content information of each node. The model is trained jointly to optimize for the task of node classification as well as the task of predicting graph context. Experimental results show that GAT-POS reaches remarkable improvement compared to strong GNN baselines and recent structural embedding enhanced GNNs on non-homophilic graphs.

==> sections/supple.tex <==
\begin{tabular}{llll}
\toprule
{} &            Cora &        Citeseer &          Pubmed \\
model          &                 &                 &                 \\
\midrule
GeomGCN-g-I    &  85.81\% (1.50\%) &  80.05\% (1.59\%) &  92.56\% (0.33\%) \\
GeomGCN-g-P    &  86.48\% (1.49\%) &  75.74\% (1.58\%) &  88.49\% (0.56\%) \\
GeomGCN-g-S    &  86.50\% (1.43\%) &  75.91\% (2.26\%) &  88.55\% (0.53\%) \\
GAT-POS-C-GS   &  87.31\% (1.40\%) &  74.71\% (1.33\%) &  85.11\% (2.57\%) \\
GAT-POS-C-PI   &  87.29\% (1.52\%) &  74.67\% (1.31\%) &  85.10\% (2.57\%) \\
GAT-POS-C-PT   &  86.61\% (1.13\%) &  73.81\% (1.27\%) &  85.09\% (2.57\%) \\
GAT-POS-T-GS   &  87.90\% (0.97\%) &  75.30\% (1.10\%) &  86.57\% (1.73\%) \\
GAT-POS-T-PI   &  85.90\% (1.47\%) &  72.88\% (1.98\%) &  85.70\% (0.94\%) \\
GAT-POS-T-PT   &  82.32\% (1.75\%) &  66.68\% (2.01\%) &  83.73\% (1.21\%) \\
GAT-POS-CG-GS  &  87.01\% (1.64\%) &  74.70\% (1.31\%) &  85.12\% (2.56\%) \\
GAT-POS-CML-PI &  87.60\% (1.69\%) &  74.77\% (1.34\%) &  85.09\% (2.59\%) \\
GAT-POS-CML-PT &  86.25\% (1.29\%) &  74.65\% (2.01\%) &  85.50\% (2.14\%) \\
\bottomrule
\end{tabular}





\begin{tabular}{llll}
\toprule
{} &       Chameleon &        Squirrel &           Actor \\
model          &                 &                 &                 \\
\midrule
GeomGCN-g-I    &  61.97\% (2.01\%) &  39.91\% (1.77\%) &  32.98\% (0.78\%) \\
GeomGCN-g-P    &  60.31\% (2.07\%) &  37.14\% (1.19\%) &  31.60\% (1.06\%) \\
GeomGCN-g-S    &  63.86\% (1.78\%) &  42.73\% (2.16\%) &  31.96\% (1.97\%) \\
GAT-POS-C-GS   &  64.39\% (2.16\%) &  43.56\% (3.15\%) &  34.78\% (1.00\%) \\
GAT-POS-C-PI   &  67.65\% (2.82\%) &  42.58\% (1.66\%) &  34.65\% (1.21\%) \\
GAT-POS-C-PT   &  67.76\% (2.54\%) &  52.90\% (1.55\%) &  34.89\% (1.38\%) \\
GAT-POS-T-GS   &  65.99\% (2.66\%) &  47.79\% (2.16\%) &  34.75\% (1.16\%) \\
GAT-POS-T-PI   &  63.79\% (2.35\%) &  47.96\% (3.29\%) &  34.59\% (1.01\%) \\
GAT-POS-T-PT   &  65.55\% (2.38\%) &  51.62\% (1.84\%) &  31.97\% (1.27\%) \\
GAT-POS-CG-GS  &  65.92\% (2.29\%) &  48.39\% (1.61\%) &  34.89\% (1.08\%) \\
GAT-POS-CML-PI &  66.67\% (2.15\%) &  47.44\% (2.33\%) &  34.98\% (1.04\%) \\
GAT-POS-CML-PT &  67.48\% (3.08\%) &  50.94\% (2.77\%) &  35.03\% (1.44\%) \\
\bottomrule
\end{tabular}












